TESS-Keck Survey XIV: Two giant exoplanets from the Distant Giants Survey

We present the Distant Giants Survey, a three-year radial velocity (RV) campaign to measure P(DG|CS), the conditional occurrence of distant giant planets (DG; M_p ~ 0.3 - 13 M_J, P > 1 year) in systems hosting a close-in small planet (CS; R_p < 10 R_E). For the past two years, we have monitored 47 Sun-like stars hosting small transiting planets detected by TESS. We present the selection criteria used to assemble our sample and report the discovery of two distant giant planets, TOI-1669 b and TOI-1694 c. For TOI-1669 b we find that Msin i = 0.573 +/- 0.074 M_J, P = 502 +/- 16 days, and e < 0.27, while for TOI-1694 c, Msin i = 1.05 +/- 0.05 M_J, P = 389.2 +/- 3.9 days, and e = 0.18 +/- 0.05. We also confirmed the 3.8-day transiting planet TOI-1694 b by measuring a true mass of M = 26.1 +/- 2.2 M_E. We also confirmed the 3.8-day transiting planet TOI-1694 b by measuring a true mass of M = 26.1 +/- 2.2 M_E. At the end of the Distant Giants Survey, we will incorporate TOI-1669 b and TOI-1694 c into our calculation of P(DG|CS), a crucial statistic for understanding the relationship between outer giants and small inner companions.

==> contrast_curve_test.tex <==
\begin{deluxetable*}{lrcrrrrrrrrrrrr}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{Detection Limits for Targets Observed at Keck with NIRC2 Imaging}
\tablehead{
\colhead{Name} & \colhead{Epoch} & \colhead{Filter+} & \colhead{$N_{obs}$} & \colhead{$t_{int}$} &  \multicolumn{10}{c}{Contrast $\Delta m$ (mag) at $\rho = $ (mas)}
\\
\colhead{} & \colhead{(MJD)} & \colhead{Coronagraph} & \colhead{} & \colhead{(sec)} & \colhead{150} & \colhead{200} & \colhead{250} & \colhead{300} & \colhead{400} & \colhead{500} & \colhead{700} & \colhead{1000} & \colhead{1500} & \colhead{2000}
}
\startdata
            TOI-1438 & 59766.40 &   Kp     &  4 &   80.00 &  4.1 &  4.7 &  5.4 &  6.1 &  6.8 &  7.1 &  7.6 &  7.9 &  7.9 &  8.0 \\ % N2.20220706.34316
\enddata
\tablecomments{}
\end{deluxetable*}
